Modeling Player and Team Performance in Basketball

In recent years, analytics has started to revolutionize the game of basketball: quantitative analyses of the game inform team strategy, management of player health and fitness, and how teams draft, sign, and trade players. In this review, we focus on methods for quantifying and characterizing basketball gameplay. At the team level, we discuss methods for characterizing team strategy and performance, while at the player level, we take a deep look into a myriad of tools for player evaluation. This includes metrics for overall player value, defensive ability, and shot modeling, and methods for understanding performance over multiple seasons via player production curves. We conclude with a discussion on the future of basketball analytics, and in particular highlight the need for causal inference in sports.

==> abstract_content.tex <==
The development of analytical tools for use in basketball has a rich and growing history.

Basketball has experienced a surge of interest in recent years

The use of analytics in basketball has grown significantly in the past fifteen years. The increase in statistical methods can be traced to a burgeoning interest in the game along with a growing availability of basketball data. In this review, we highlight interesting methods developed to model the game of basketball 

% this one is the abstract:
For basketball in particular, a rise in data availability -- including tracking data, where players and the ball are tracked through space and time -- has led to the development of new statistical methods for understanding the game. In this review, we discuss methods for modeling basketball gameplay on both the team-level and the player-level. At the team level, we focus on characterizing strategies and team performance, while at the player level, we take a deep look into a myriad of tools for player evaluation. This includes metrics for overall player value, defensive ability, shot modeling, and in understanding performance over multiple seasons via player production curves. We conclude with a discussion on the future of basketball analytics, and in particular highlight the need for more causal analyses.

==> bib.tex <==
\begin{thebibliography}{}

\bibitem{bbref_bpm}
About box plus/minus ({BPM}).
\newblock https://www.basketball-reference.com/about/bpm2.html.

\bibitem{bbref_ratings}
Calculating individual offensive and defensive ratings.
\newblock https://www.basketball-reference.com/about/ratings.html.

\bibitem{nbastats}
{NBA} {S}tats.
\newblock https://stats.nba.com/.

\bibitem{nfl_football_operations}
{NFL} big data bowl.
\newblock https://operations.nfl.com/the-game/big-data-bowl/.

\bibitem{rspct}
{RSPCT}.
\newblock https://www.rspctbasketball.com/.

\bibitem{alferink2009generality}
Larry~A Alferink, Thomas~S Critchfield, Jennifer~L Hitt, and William~J Higgins.
\newblock Generality of the matching law as a descriptor of shot selection in
  basketball.
\newblock {\em Journal of Applied Behavior Analysis}, 42(3):595--608, 2009.

\bibitem{arkes2010revisiting}
Jeremy Arkes.
\newblock Revisiting the hot hand theory with free throw data in a multivariate
  framework.
\newblock {\em Journal of Quantitative Analysis in Sports}, 6(1), 2010.

\bibitem{bar2006twenty}
Michael Bar-Eli, Simcha Avugos, and Markus Raab.
\newblock Twenty years of “hot hand” research: Review and critique.
\newblock {\em Psychology of Sport and Exercise}, 7(6):525--553, 2006.

\bibitem{berri1999most}
David~J Berri.
\newblock Who is ‘most valuable’? measuring the player's production of wins
  in the national basketball association.
\newblock {\em Managerial and decision economics}, 20(8):411--427, 1999.

\bibitem{blei2003latent}
David~M. Blei, Andrew~Y. Ng, and Michael~I. Jordan.
\newblock Latent {D}irichlet allocation.
\newblock {\em The Journal of Machine Learning Research}, 3:993--1022, 2003.

\bibitem{bornn2017studying}
Luke Bornn, Daniel Cervone, Alexander Franks, and Andrew Miller.
\newblock Studying basketball through the lens of player tracking data.
\newblock In {\em Handbook of Statistical Methods and Analyses in Sports},
  pages 261--286. Chapman and Hall/CRC, 2017.

\bibitem{bornn2019using}
Luke Bornn and Daniel Daly-Grafstein.
\newblock Using in-game shot trajectories to better understand defensive impact
  in the nba.
\newblock {\em arXiv preprint arXiv:1905.00822}, 2019.

\bibitem{brown2012insights}
Mark Brown, Paul Kvam, George Nemhauser, and Joel Sokol.
\newblock Insights from the lrmc method for {NCAA} tournament predictions.
\newblock MIT Sloan Sports Conference, 2012.

\bibitem{brown2010improved}
Mark Brown and Joel Sokol.
\newblock An improved lrmc method for {NCAA} basketball prediction.
\newblock {\em Journal of Quantitative Analysis in Sports}, 6(3), 2010.

\bibitem{brown1993fundamentals}
William~O Brown and Raymond~D Sauer.
\newblock Fundamentals or noise? evidence from the professional basketball
  betting market.
\newblock {\em The Journal of Finance}, 48(4):1193--1209, 1993.

\bibitem{carlin1994improved}
Bradley~P Carlin.
\newblock Improved {NCAA} basketball tournament modeling via point spread and
  team strength information.
\newblock In {\em Anthology of Statistics in Sports}, pages 149--153. SIAM,
  2005.

\bibitem{cervone2016nba}
Dan Cervone, Luke Bornn, and Kirk Goldsberry.
\newblock Nba court realty.
\newblock In {\em 10th MIT Sloan Sports Analytics Conference}, 2016.

\bibitem{cervonepointwise}
Dan Cervone, Alexander D'Amour, Luke Bornn, and Kirk Goldsberry.
\newblock Pointwise: Predicting points and valuing decisions in real time with
  {NBA} optical tracking data.
\newblock 2014.

\bibitem{cervone2014multiresolution}
Daniel Cervone, Alex D'Amour, Luke Bornn, and Kirk Goldsberry.
\newblock A multiresolution stochastic process model for predicting basketball
  possession outcomes.
\newblock {\em arXiv preprint arXiv:1408.0777}, 2014.

\bibitem{chang2014quantifying}
Yu-Han Chang, Rajiv Maheswaran, Jeff Su, Sheldon Kwok, Tal Levy, Adam Wexler,
  and Kevin Squire.
\newblock Quantifying shot quality in the {NBA}.
\newblock In {\em Proceedings of the 8th Annual MIT Sloan Sports Analytics
  Conference. MIT, Boston, MA}, 2014.

\bibitem{csapo2014hand}
Peter Csapo and Markus Raab.
\newblock “hand down, man down.” analysis of defensive adjustments in
  response to the hot hand in basketball using novel defense metrics.
\newblock {\em PloS one}, 9(12):e114184, 2014.

\bibitem{daly2019rao}
Daniel Daly-Grafstein and Luke Bornn.
\newblock Rao-blackwellizing field goal percentage.
\newblock {\em Journal of Quantitative Analysis in Sports}, 15(2):85--95, 2019.

\bibitem{deshpande2016estimating}
Sameer~K Deshpande and Shane~T Jensen.
\newblock Estimating an {NBA} player’s impact on his team’s chances of
  winning.
\newblock {\em Journal of Quantitative Analysis in Sports}, 12(2):51--72, 2016.

\bibitem{difiori2018nba}
John~P DiFiori, Arne G{\"u}llich, Joel~S Brenner, Jean C{\^o}t{\'e}, Brian
  Hainline, Edward Ryan, and Robert~M Malina.
\newblock The {NBA} and youth basketball: recommendations for promoting a
  healthy and positive experience.
\newblock {\em Sports Medicine}, 48(9):2053--2065, 2018.

\bibitem{drakos2010injury}
Mark~C Drakos, Benjamin Domb, Chad Starkey, Lisa Callahan, and Answorth~A
  Allen.
\newblock Injury in the national basketball association: a 17-year overview.
\newblock {\em Sports health}, 2(4):284--290, 2010.

\bibitem{drazan2017sports}
John~F Drazan, Amy~K Loya, Benjamin~D Horne, and Ron Eglash.
\newblock From sports to science: Using basketball analytics to broaden the
  appeal of math and science among youth.
\newblock In {\em MIT-Sloan Sport. Anal. Conf.}, pages 1--16, 2017.

\bibitem{dutta2017identifying}
Shouvik Dutta, Sheldon~H Jacobson, and Jason~J Sauppe.
\newblock Identifying {NCAA} tournament upsets using balance optimization
  subset selection.
\newblock {\em Journal of Quantitative Analysis in Sports}, 13(2):79--93, 2017.

\bibitem{d2015move}
Alexander D’Amour, Daniel Cervone, Luke Bornn, and Kirk Goldsberry.
\newblock Move or die: How ball movement creates open shots in the {NBA}.
\newblock Boston, MA: MIT Sloan Sports Analytics Conference, 2015.

\bibitem{efron1975data}
Bradley Efron and Carl Morris.
\newblock Data analysis using stein's estimator and its generalizations.
\newblock {\em Journal of the American Statistical Association},
  70(350):311--319, 1975.

\bibitem{engelmann2017possession}
Jeremias Engelmann.
\newblock Possession-based player performance analysis in basketball
  (adjusted+/--and related concepts).
\newblock In {\em Handbook of Statistical Methods and Analyses in Sports},
  pages 231--244. Chapman and Hall/CRC, 2017.

\bibitem{espnmac}
ESPN.
\newblock 5-on-5: Can {L}e{B}ron catch {G}iannis for {MVP}?, Feb 2020.

\bibitem{fearnhead2011estimating}
Paul Fearnhead and Benjamin~Matthew Taylor.
\newblock On estimating the ability of {NBA} players.
\newblock {\em Journal of quantitative analysis in sports}, 7(3), 2011.

\bibitem{fewell2012basketball}
Jennifer~H Fewell, Dieter Armbruster, John Ingraham, Alexander Petersen, and
  James~S Waters.
\newblock Basketball teams as strategic networks.
\newblock {\em PloS one}, 7(11):e47445, 2012.

\bibitem{franks2015counterpoints}
Alexander Franks, Andrew Miller, Luke Bornn, and Kirk Goldsberry.
\newblock Counterpoints: Advanced defensive metrics for {NBA} basketball.
\newblock In {\em 9th Annual MIT Sloan Sports Analytics Conference, Boston,
  MA}, 2015.

\bibitem{franks2015characterizing}
Alexander Franks, Andrew Miller, Luke Bornn, Kirk Goldsberry, et~al.
\newblock Characterizing the spatial structure of defensive skill in
  professional basketball.
\newblock {\em The Annals of Applied Statistics}, 9(1):94--121, 2015.

\bibitem{franks2016meta}
Alexander~M Franks, Alexander D’Amour, Daniel Cervone, and Luke Bornn.
\newblock Meta-analytics: tools for understanding the statistical properties of
  sports metrics.
\newblock {\em Journal of Quantitative Analysis in Sports}, 12(4):151--165,
  2016.

\bibitem{gandar1998informed}
John~M Gandar, William~H Dare, Craig~R Brown, and Richard~A Zuber.
\newblock Informed traders and price variations in the betting market for
  professional basketball games.
\newblock {\em The Journal of Finance}, 53(1):385--401, 1998.

\bibitem{gauriot2018fooled}
Romain Gauriot and Lionel Page.
\newblock Fooled by performance randomness: over-rewarding luck.
\newblock {\em Review of Economics and Statistics}, (0), 2018.

\bibitem{gilovich1985hot}
Thomas Gilovich, Robert Vallone, and Amos Tversky.
\newblock The hot hand in basketball: On the misperception of random sequences.
\newblock {\em Cognitive psychology}, 17(3):295--314, 1985.

\bibitem{glickman2015introduction}
Mark~E Glickman and Jeff Sonas.
\newblock Introduction to the {NCAA} men’s basketball prediction methods
  issue.
\newblock {\em Journal of Quantitative Analysis in Sports}, 11(1):1--3, 2015.

\bibitem{goldman2011allocative}
Matt Goldman and Justin~M Rao.
\newblock Allocative and dynamic efficiency in {NBA} decision making.
\newblock In {\em In Proceedings of the MIT Sloan Sports Analytics Conference},
  pages 4--5, 2011.

\bibitem{goldman2013live}
Matthew Goldman and Justin~M Rao.
\newblock Live by the three, die by the three? the price of risk in the nba.
\newblock In {\em Submission to the MIT Sloan Sports Analytics Conference},
  2013.

\bibitem{goldsberry2012courtvision}
Kirk Goldsberry.
\newblock Courtvision: New visual and spatial analytics for the {NBA}.
\newblock MIT Sloan Sports Analytics Conference 2012, 2012.

\bibitem{goldsberry2019sprawlball}
Kirk Goldsberry.
\newblock {\em Sprawlball : a visual tour of the new era of the NBA}.
\newblock Houghton Mifflin Harcourt, Boston, 2019.

\bibitem{goldsberry2013dwight}
Kirk Goldsberry and Eric Weiss.
\newblock The dwight effect: A new ensemble of interior defense analytics for
  the {NBA}.
\newblock {\em Sports Aptitude, LLC. Web}, pages 1--11, 2013.

\bibitem{gray2012comparing}
Kathy~L Gray and Neil~C Schwertman.
\newblock Comparing team selection and seeding for the 2011 {NCAA} men's
  basketball tournament.
\newblock {\em Journal of Quantitative Analysis in Sports}, 8(1), 2012.

\bibitem{gupta2015new}
Ajay~Andrew Gupta.
\newblock A new approach to bracket prediction in the {NCAA} men’s basketball
  tournament based on a dual-proportion likelihood.
\newblock {\em Journal of Quantitative Analysis in Sports}, 11(1):53--67, 2015.

\bibitem{harmon2016predicting}
Mark Harmon, Patrick Lucey, and Diego Klabjan.
\newblock Predicting shot making in basketball using convolutional neural
  networks learnt from adversarial multiagent trajectories.
\newblock {\em stat}, 1050:15, 2016.

\bibitem{hofler2006efficiency}
Richard~A Hofler and James~E Payne.
\newblock Efficiency in the national basketball association: a stochastic
  frontier approach with panel data.
\newblock {\em Managerial and Decision Economics}, 27(4):279--285, 2006.

\bibitem{hollinger2004pro}
J.~Hollinger.
\newblock {\em Pro Basketball Forecast, 2005-06}.
\newblock Potomac Books, Washington, D.C, 2005.

\bibitem{hollingerper}
John Hollinger.
\newblock Per: Player efficiency rating explained, Aug 2005.

\bibitem{hughes_2017}
Grant Hughes.
\newblock How europe changed the {NBA} game forever, Oct 2017.

\bibitem{noah}
Noah Basketball Pillar~Vision Inc.
\newblock Noah basketball.

\bibitem{jacobs_2017}
Jordan Jacobs.
\newblock Deep dive on regularized adjusted plus-minus i: Introductory example,
  Sep 2017.

\bibitem{james1984the-bill}
Bill James.
\newblock {\em The Bill James Baseball Abstract, 1984}.
\newblock Ballantine Books New York, 1984.

\bibitem{james1987bill}
Bill James.
\newblock {\em The Bill James Baseball Abstract 1987}.
\newblock Ballantine Books, 1987.

\bibitem{james2010new}
Bill James.
\newblock {\em The new Bill James historical baseball abstract}.
\newblock Simon and Schuster, 2010.

\bibitem{keshri2019automatic}
Suraj Keshri, Min-hwan Oh, Sheng Zhang, and Garud Iyengar.
\newblock Automatic event detection in basketball using hmm with energy based
  defensive assignment.
\newblock {\em Journal of Quantitative Analysis in Sports}, 15(2):141--153,
  2019.

\bibitem{kubatko2007starting}
Justin Kubatko, Dean Oliver, Kevin Pelton, and Dan~T RoseNBAum.
\newblock A starting point for analyzing basketball statistics.
\newblock {\em Journal of Quantitative Analysis in Sports}, 3(3), 2007.

\bibitem{kvam2006logistic}
Paul Kvam and Joel~S Sokol.
\newblock A logistic regression/markov chain model for {NCAA} basketball.
\newblock {\em Naval Research Logistics (NrL)}, 53(8):788--803, 2006.

\bibitem{lackritz2017probability}
James Lackritz.
\newblock Probability models for streak shooting.
\newblock In {\em Handbook of Statistical Methods and Analyses in Sports},
  pages 215--230. Chapman and Hall/CRC, 2017.

\bibitem{lamas2015modeling}
Leonardo Lamas, Felipe Santana, Matthew Heiner, Carlos Ugrinowitsch, and
  Gilbert Fellingham.
\newblock Modeling the offensive-defensive interaction and resulting outcomes
  in basketball.
\newblock {\em PloS one}, 10(12):e0144435, 2015.

\bibitem{le2017data}
Hoang~M Le, Peter Carr, Yisong Yue, and Patrick Lucey.
\newblock Data-driven ghosting using deep imitation learning.
\newblock 2017.

\bibitem{lewis2004moneyball}
Michael Lewis.
\newblock {\em Moneyball: The art of winning an unfair game}.
\newblock WW Norton \& Company, 2004.

\bibitem{github-tracking}
linouk23.
\newblock linouk23/nba-player-movements, Sep 2016.

\bibitem{lopez2016persuaded}
Michael~J Lopez.
\newblock Persuaded under pressure: Evidence from the national football league.
\newblock {\em Economic Inquiry}, 54(4):1763--1773, 2016.

\bibitem{lopez2015building}
Michael~J Lopez and Gregory~J Matthews.
\newblock Building an {NCAA} men’s basketball predictive model and
  quantifying its success.
\newblock {\em Journal of Quantitative Analysis in Sports}, 11(1):5--12, 2015.

\bibitem{lucey2014get}
Patrick Lucey, Alina Bialkowski, Peter Carr, Yisong Yue, and Iain Matthews.
\newblock How to get an open shot: Analyzing team movement in basketball using
  tracking data.
\newblock In {\em Proceedings of the 8th annual MIT SLOAN sports analytics
  conference}, 2014.

\bibitem{malarranha2013dynamic}
Jorge Malarranha, Bruno Figueira, Nuno Leite, and Jaime Sampaio.
\newblock Dynamic modeling of performance in basketball.
\newblock {\em International Journal of Performance Analysis in Sport},
  13(2):377--387, 2013.

\bibitem{marty2018high}
Rachel Marty.
\newblock High-resolution shot capture reveals systematic biases and an
  improved method for shooter evalutation.
\newblock In {\em Proceedings of the 2018 MIT Sloan Sports Analytics
  Conference}, 2018.

\bibitem{marty2017data}
Rachel Marty and Simon Lucey.
\newblock A data-driven method for understanding and increasing 3-point
  shooting percentage.
\newblock In {\em Proceedings of the 2017 MIT Sloan Sports Analytics
  Conference}, 2017.

\bibitem{masheswaran2014three}
R~Masheswaran, Y~Chang, Jeff Su, Sheldon Kwok, Tal Levy, Adam Wexler, and Noel
  Hollingsworth.
\newblock The three dimensions of rebounding.
\newblock {\em MIT SSAC}, 2014.

\bibitem{melnick2001relationship}
Merrill~J Melnick.
\newblock Relationship between team assists and win-loss record in the national
  basketball association.
\newblock {\em Perceptual and Motor Skills}, 92(2):595--602, 2001.

\bibitem{metulini2018modelling}
Rodolfo Metulini, Marica Manisera, and Paola Zuccolotto.
\newblock Modelling the dynamic pattern of surface area in basketball and its
  effects on team performance.
\newblock {\em Journal of Quantitative Analysis in Sports}, 14(3):117--130,
  2018.

\bibitem{miller2013icml}
A.~Miller, L.~Bornn, R.~Adams, and K.~Goldsberry.
\newblock Factorized point process intensities: A spatial analysis of
  professional basketball.
\newblock In {\em Proceedings of the 31st International Conference on Machine
  Learning}, pages 235--243. 2013.

\bibitem{miller2017possession}
Andrew~C Miller and Luke Bornn.
\newblock Possession sketches: Mapping {NBA} strategies.
\newblock In {\em MIT Sloan Sports Analytics Conference}, 2017.

\bibitem{sciam}
Joshua Miller.
\newblock Momentum isn't magic-vindicating the hot hand with the mathematics of
  streaks, Mar 2018.

\bibitem{miller2017bridge}
Joshua~B Miller and Adam Sanjurjo.
\newblock A bridge from monty hall to the hot hand: Restricted choice,
  selection bias, and empirical practice.
\newblock 2017.

\bibitem{miller2015surprised}
Joshua~B Miller, Adam Sanjurjo, et~al.
\newblock Surprised by the gambler’s and hot hand fallacies.
\newblock {\em A truth in the law of small numbers}, 2015.

\bibitem{myers}
Daniel Myers.
\newblock About box plus/minus ({BPM}).

\bibitem{nba_glossary}
{N}ational~{B}asketball {A}ssociation.
\newblock A glossary of {NBA} terms.
\newblock {http://www.NBA.com/analysis/00422966.html}, 2014.

\bibitem{neiman2011reinforcement}
Tal Neiman and Yonatan Loewenstein.
\newblock Reinforcement learning in professional basketball players.
\newblock {\em Nature communications}, 2(1):1--8, 2011.

\bibitem{neudorfer2018predicting}
Ayala Neudorfer and Saharon Rosset.
\newblock Predicting the {NCAA} basketball tournament using isotonic least
  squares pairwise comparison model.
\newblock {\em Journal of Quantitative Analysis in Sports}, 14(4):173--183,
  2018.

\bibitem{oliver2004basketball}
Dean Oliver.
\newblock {\em Basketball on paper: rules and tools for performance analysis}.
\newblock Potomac Books, Inc., 2004.

\bibitem{omidiran2011pm}
D.~Omidiran.
\newblock A new look at adjusted plus/minus for basketball analysis.
\newblock {\em MIT Sloan Sports Analytics Conference [online]}, 2011, 2011.

\bibitem{page2013effect}
Garritt~L Page, Bradley~J Barney, and Aaron~T McGuire.
\newblock Effect of position, usage rate, and per game minutes played on {NBA}
  player production curves.
\newblock {\em Journal of Quantitative Analysis in Sports}, 9(4):337--345,
  2013.

\bibitem{page2007using}
Garritt~L Page, Gilbert~W Fellingham, and C~Shane Reese.
\newblock Using box-scores to determine a position's contribution to winning
  basketball games.
\newblock {\em Journal of Quantitative Analysis in Sports}, 3(4), 2007.

\bibitem{visualizegravity}
Andrew Patton.
\newblock How can we visualize a player’s shooting gravity?
\newblock
  \url{https://fansided.com/2019/07/22/nylon-calculus-visualizing-NBA-shooting-gravity/},
  2014.
\newblock Accessed: 2019-07-23.

\bibitem{pelton}
Kevin Pelton.
\newblock The warp rating system explained.

\bibitem{pesca_2009}
Mike Pesca.
\newblock The man who made baseball's box score a hit, Jul 2009.

\bibitem{piette2011evaluating}
James Piette, Lisa Pham, and Sathyanarayan Anand.
\newblock Evaluating basketball player performance via statistical network
  modeling.
\newblock In {\em MIT Sloan Sports Anal. Conf.}, 2011.

\bibitem{poling2011matching}
Alan Poling, Timothy~L Edwards, Marc Weeden, and T~Mary Foster.
\newblock The matching law.
\newblock {\em The Psychological Record}, 61(2):313--322, 2011.

\bibitem{prentice1979hazard}
Ross~L Prentice and John~D Kalbfleisch.
\newblock Hazard rate models with covariates.
\newblock {\em Biometrics}, pages 25--39, 1979.

\bibitem{price2010racial}
Joseph Price and Justin Wolfers.
\newblock Racial discrimination among {NBA} referees.
\newblock {\em The Quarterly journal of economics}, 125(4):1859--1887, 2010.

\bibitem{reich2006spatial}
Brian~J Reich, James~S Hodges, Bradley~P Carlin, and Adam~M Reich.
\newblock A spatial analysis of basketball shot chart data.
\newblock {\em The American Statistician}, 60(1):3--12, 2006.

\bibitem{rosenbaum}
Dan~T Rosenbaum.
\newblock Measuring how {NBA} players help their teams win.
\newblock {\em 82Games. com (http://www.82games.com/comm30. htm)}, pages 4--30,
  2004.

\bibitem{ruiz2015generative}
Francisco~JR Ruiz and Fernando Perez-Cruz.
\newblock A generative model for predicting outcomes in college basketball.
\newblock {\em Journal of Quantitative Analysis in Sports}, 11(1):39--52, 2015.

\bibitem{sampaio2003statistical}
Jaime Sampaio and Manuel Janeira.
\newblock Statistical analyses of basketball team performance: understanding
  teams’ wins and losses according to a different index of ball possessions.
\newblock {\em International Journal of Performance Analysis in Sport},
  3(1):40--49, 2003.

\bibitem{simpsons_personal}
Nathan Sandholtz and Luke Bornn.
\newblock Personal communication, 2017.

\bibitem{sandholtz2018transition}
Nathan Sandholtz and Luke Bornn.
\newblock Transition tensor markov decision processes: Analyzing shot policies
  in professional basketball.
\newblock {\em arXiv preprint arXiv:1812.05170}, 2018.

\bibitem{sandholtz2019measuring}
Nathan Sandholtz, Jacob Mortensen, and Luke Bornn.
\newblock Measuring spatial allocative efficiency in basketball.
\newblock {\em arXiv preprint arXiv:1912.05129}, 2019.

\bibitem{schwartz_2013}
Jason Schwartz.
\newblock The {NBA} loves stats. that's a problem., Feb 2013.

\bibitem{schwertman1991probability}
Neil~C Schwertman, Thomas~A McCready, and Lesley Howard.
\newblock Probability models for the {NCAA} regional basketball tournaments.
\newblock {\em The American Statistician}, 45(1):35--38, 1991.

\bibitem{schwertman1996more}
Neil~C Schwertman, Kathryn~L Schenk, and Brett~C Holbrook.
\newblock More probability models for the {NCAA} regional basketball
  tournaments.
\newblock {\em The American Statistician}, 50(1):34--38, 1996.

\bibitem{shah2016applying}
Rajiv Shah and Rob Romijnders.
\newblock Applying deep learning to basketball trajectories.
\newblock {\em arXiv preprint arXiv:1608.03793}, 2016.

\bibitem{shortridge2014creating}
Ashton Shortridge, Kirk Goldsberry, and Matthew Adams.
\newblock Creating space to shoot: quantifying spatial relative field goal
  efficiency in basketball.
\newblock {\em Journal of Quantitative Analysis in Sports}, 10(3):303--313,
  2014.

\bibitem{sicilia2019deephoops}
Anthony Sicilia, Konstantinos Pelechrinis, and Kirk Goldsberry.
\newblock Deephoops: Evaluating micro-actions in basketball using deep feature
  representations of spatio-temporal data.
\newblock {\em arXiv preprint arXiv:1902.08081}, 2019.

\bibitem{sill2010improved}
Joseph Sill.
\newblock Improved {NBA} adjusted plus-minus using regularization and
  out-of-sample testing.
\newblock In {\em Proceedings of the 2010 MIT Sloan Sports Analytics
  Conference}, 2010.

\bibitem{silver2012signal}
Nate Silver.
\newblock {\em The signal and the noise: why so many predictions fail--but some
  don't}.
\newblock Penguin, 2012.

\bibitem{natesilver538_2015}
Nate Silver.
\newblock We're predicting the career of every {NBA} player. {H}ere's how., Oct
  2015.

\bibitem{natesilver538_2019}
Nate Silver.
\newblock How our {RAPTOR} metric works, Oct 2019.

\bibitem{simmons}
Bill Simmons.
\newblock Ewing {T}heory 101.
\newblock https://www.espn.com/espn/page2/story?page=simmons/010509a.

\bibitem{skinner2010price}
Brian Skinner.
\newblock The price of anarchy in basketball.
\newblock {\em Journal of Quantitative Analysis in Sports}, 6(1), 2010.

\bibitem{skinner2015optimal}
Brian Skinner and Matthew Goldman.
\newblock Optimal strategy in basketball.
\newblock {\em arXiv preprint arXiv:1512.05652}, 2015.

\bibitem{skinner2015method}
Brian Skinner and Stephen~J Guy.
\newblock A method for using player tracking data in basketball to learn player
  skills and predict team performance.
\newblock {\em PloS one}, 10(9):e0136393, 2015.

\bibitem{smith_2018}
Chris Smith.
\newblock Kinexon's wearable sensor is changing the way {NBA} teams prep for
  success, Nov 2018.

\bibitem{stone2012measurement}
Daniel~F Stone.
\newblock Measurement error and the hot hand.
\newblock {\em The American Statistician}, 66(1):61--66, 2012.

\bibitem{tu2008simpson}
Yu-Kang Tu, David Gunnell, and Mark~S Gilthorpe.
\newblock Simpson's paradox, lord's paradox, and suppression effects are the
  same phenomenon--the reversal paradox.
\newblock {\em Emerging themes in epidemiology}, 5(1):2, 2008.

\bibitem{vaci2019large}
Nemanja Vaci, Dijana Coci{\'c}, Bartosz Gula, and Merim Bilali{\'c}.
\newblock Large data and bayesian modeling—aging curves of {NBA} players.
\newblock {\em Behavior research methods}, pages 1--21, 2019.

\bibitem{van2017adjusting}
Matthew van Bommel and Luke Bornn.
\newblock Adjusting for scorekeeper bias in {NBA} box scores.
\newblock {\em Data Mining and Knowledge Discovery}, 31(6):1622--1642, 2017.

\bibitem{vinue2019forecasting}
Guillermo Vinu{\'e} and Irene Epifanio.
\newblock Forecasting basketball players' performance using sparse functional
  data.
\newblock {\em Statistical Analysis and Data Mining: The ASA Data Science
  Journal}, 2019.

\bibitem{vinue2015archetypoids}
Guillermo Vinu{\'e}, Irene Epifanio, and Sandra Alemany.
\newblock Archetypoids: A new approach to define representative archetypal
  data.
\newblock {\em Computational Statistics \& Data Analysis}, 87:102--115, 2015.

\bibitem{wakim2014functional}
Alexander Wakim and Jimmy Jin.
\newblock Functional data analysis of aging curves in sports.
\newblock {\em arXiv preprint arXiv:1403.7548}, 2014.

\bibitem{xin2017continuous}
Lu~Xin, Mu~Zhu, Hugh Chipman, et~al.
\newblock A continuous-time stochastic block model for basketball networks.
\newblock {\em The Annals of Applied Statistics}, 11(2):553--597, 2017.

\bibitem{yaari2011hot}
Gur Yaari and Shmuel Eisenmann.
\newblock The hot (invisible?) hand: can time sequence patterns of
  success/failure in sports be modeled as repeated random independent trials?
\newblock {\em PloS one}, 6(10):e24532, 2011.

\bibitem{yamlost}
Derrick~R Yam and Michael~J Lopez.
\newblock What was lost? a causal estimate of fourth down behavior in the
  national football league.
\newblock {\em Journal of Sports Analytics}, (Preprint):1--15.

\bibitem{yu2010hidden}
Shun-Zheng Yu.
\newblock Hidden semi-markov models.
\newblock {\em Artificial Intelligence}, 174(2):215--243, 2010.

\bibitem{yuan2015mixture}
Lo-Hua Yuan, Anthony Liu, Alec Yeh, Aaron Kaufman, Andrew Reece, Peter Bull,
  Alex Franks, Sherrie Wang, Dmitri Illushin, and Luke Bornn.
\newblock A mixture-of-modelers approach to forecasting {NCAA} tournament
  outcomes.
\newblock {\em Journal of Quantitative Analysis in Sports}, 11(1):13--27, 2015.

\bibitem{yue2014learning}
Yisong Yue, Patrick Lucey, Peter Carr, Alina Bialkowski, and Iain Matthews.
\newblock Learning fine-grained spatial models for dynamic sports play
  prediction.
\newblock In {\em 2014 IEEE international conference on data mining}, pages
  670--679. IEEE, 2014.

\bibitem{ziv2010predicting}
Gal Ziv, Ronnie Lidor, and Michal Arnon.
\newblock Predicting team rankings in basketball: The questionable use of
  on-court performance statistics.
\newblock {\em International Journal of Performance Analysis in Sport},
  10(2):103--114, 2010.

\bibitem{zuccolotto2018big}
Paola Zuccolotto, Marica Manisera, and Marco Sandri.
\newblock Big data analytics for modeling scoring probability in basketball:
  The effect of shooting under high-pressure conditions.
\newblock {\em International Journal of Sports Science \& Coaching},
  13(4):569--589, 2018.

\end{thebibliography}

